Is DPO Superior to PPO for LLM Alignment? A Comprehensive Study

Reinforcement Learning from Human Feedback (RLHF) is currently the most widely used method to align large language models (LLMs) with human preferences. Existing RLHF methods can be roughly categorized as either reward-based or reward-free. Novel applications such as ChatGPT and Claude leverage reward-based methods that first learn a reward model and apply actor-critic algorithms, such as Proximal Policy Optimization (PPO). However, in academic benchmarks, state-of-the-art results are often achieved via reward-free methods, such as Direct Preference Optimization (DPO). Is DPO truly superior to PPO? Why does PPO perform poorly on these benchmarks? In this paper, we first conduct both theoretical and empirical studies on the algorithmic properties of DPO and show that DPO may have fundamental limitations. Moreover, we also comprehensively examine PPO and reveal the key factors for the best performances of PPO in fine-tuning LLMs. Finally, we benchmark DPO and PPO across a collection of RLHF testbeds, ranging from dialogue to code generation. Experiment results demonstrate that PPO is able to surpass other alignment methods in all cases and achieve state-of-the-art results in challenging code competitions. Our code is publicly available at https://github.com/openpsi-project/ReaLHF.

==> _proofs.tex <==
\section{Proofs}
\label{app:proof}

% Without the loss of generality, we assume a fixed vocabulary size, a maximum length of prompts $H_\mathrm{prompt}$, and a maximum length of responses $H_\mathrm{resp}$, such that the spaces of prompts $\mathcal{X}$ and responses $\mathcal{Y}$ are finite sets. This is also the common practice for implementing transformer-based language models.

% \begin{definition}
% (Ranking Graph)
% The ranking graph $G(\x)$ w.r.t. a prompt $\x$ of a preference dataset $D_\mathrm{pref}=\{(\x^i,\y^i_w,\y^i_l)\}_N$ is defined by a set of nodes $\mathcal{V}$ and directional edges $\mathcal{E}(\x)$, where $\mathcal{V}=\mathcal{Y}$ is the set of all text responses and $\mathcal{E}(\x)=\{(u,v)\mid (\x,u,v)\in D_\mathrm{pref}\}$.
% \end{definition}

% \begin{definition}
% (Cyclic Ranking)
% We say a preference dataset $D_\mathrm{pref}=\{(\x^i,\y^i_w,\y^i_l)\}_N$ has \textbf{cyclic ranking} if there exists a prompt $\x$ and a cycle in its corresponding ranking graph $G(\x)$.
% \end{definition}

% \begin{definition}
% (Ranking Order)
% Given a preference dataset $D_\mathrm{pref}=\{(\x^i,\y^i_w,\y^i_l)\}_N$, a prompt $\x$, the corresponding ranking graph $G(\x)$, and two responses $\y_1$ and $\y_2$, we say the \textbf{ranking order between $\y_1$ and $\y_2$ can be inferred} if there exists a path connecting $\y_1$ and $\y_2$ in $G(\x)$.
% \end{definition}

\begin{theorem}
\label{thm:dpo}
Given preference dataset $D_\mathrm{pref}=\{(\x,\y_w,\y_l)\}_N$, denote the collection of all win/loss responses in the dataset as $\mathcal{Y}({D_\mathrm{pref}})$. 
Given a prompt $\x^\prime$,
if there exists a response $\y^\prime\notin\mathcal{Y}({D_\mathrm{pref}})$, then there exists a reward function $r^\prime$ that minimizes the loss in \cref{eq:bradley-terry}, but $r^\prime(\x^\prime,\y^\prime)$ can be arbitrarily large. 
% If there exists a response $\y^\prime$
% Denote the optimal response to a prompt $\x$ as $\y^*=\arg\max_\y r(\x,\y)$.
% Given preference dataset $D_\mathrm{pref}=\{(\x,\y_w,\y_l)\}_N$, define the reward model loss according to the Bradley-Terry model as
% \begin{equation}
%     L(r^\prime)=-\mathbb{E}_{D_\mathrm{pref}}\left[\log\sigma(r^\prime(\x,\y_w)-r^\prime(\x,\y_l))\right].
% \end{equation}
% Assume there is \textbf{no cyclic ranking} in $D_\mathrm{pref}$.
% If there exists a response $\y^\prime$, such that $r(\x,\y^\prime)<r(\x,\y^*)$ and the ranking order between $\y^*$ and $\y^\prime$ \textbf{cannot be inferred} from $D_\mathrm{pref}$, then there exists a reward model $r^\prime$, for any $\epsilon>0$, we have $L(r^\prime)<\epsilon$ and $r^\prime (\x,\y^\prime)>r^\prime(\x,\y^*)$.
\end{theorem}

\begin{proof}
From algebra we know that $-\log\sigma(r^\prime(\x,\y_w)-r^\prime(\x,\y_l))<\epsilon$ is equivalent to
\begin{equation}
    r^\prime(\x,\y_w)-r^\prime(\x,\y_l)>-\log\left(\exp(\epsilon) - 1\right)=\eta.\label{eq:rwd-less_eps}
\end{equation}
To let $L(\phi^\prime)<\epsilon$, we should ensure for any $(\x^i,\y^i_w,\y^i_l)\in D_\mathrm{pref}$, \cref{eq:rwd-less_eps} is satisfied. Next, we consider the following linear programming
\begin{align}\label{eq:rwd-lp}
    \max_{r^\prime}\,\,&r^\prime (\x,\y^\prime)- r^\prime(\x,\y^*) \\
    \mathrm{s.t.}\,\,& r^\prime(\x^i,\y_w^i)-r^\prime(\x^i,\y_l^i) > \eta, \,\,\,\,\forall (\x^i,\y^i_w,\y^i_l)\in D_\mathrm{pref}.\notag
\end{align}
% Consider $r^\prime$ to be a tabular of size $\vert\mathcal{X}\vert\times\vert\mathcal{Y}\vert$, where each number can be independently changed.
We prove that $r^\prime (\x,\y^\prime)- r^\prime(\x,\y^*)$ will not be derived in constraints of \cref{eq:rwd-lp} by contradiction. Suppose we can derive $r^\prime (\x,\y^\prime)- r^\prime(\x,\y^*)>C$ or $r^\prime (\x,\y^\prime)- r^\prime(\x,\y^*)<C$ from the constraints, then there must exist a path from $\y^\prime$ to $\y^*$ or a path from $\y^*$ to $\y^\prime$, which violates the non-cyclic and non-infer-able assumption. Therefore, $r^\prime (\x,\y^\prime)- r^\prime(\x,\y^*)$ will not be derived in the constraints of \cref{eq:rwd-lp}. As a result, $r^\prime (\x,\y^\prime)- r^\prime(\x,\y^*)$ can be arbitrarily maximized to an unbounded positive value without violating constraints.
\end{proof}

\begin{corollary}
Denote the optimal policy given by \cref{eq:obj} and \cref{eq:closeform-sol} as $\pi^*$ and a response sampled from $\pi^*(\cdot\mid\x)$ as $\y^*$.
Given preference dataset $D_\mathrm{pref}=\{(\x,\y_w,\y_l)\}_N$ and a reference model $\piref$, define the DPO loss as
\begin{equation}
    L_\mathrm{DPO}(\pi^\prime)=-\mathbb{E}_{D_\mathrm{pref}}
    \left[\log\sigma\left(\beta \log\frac{\pi^\prime(\y_w\mid\x)}{\piref(\y_w\mid\x)} -
    \beta\log\frac{\pi^\prime(\y_l\mid\x)}{\piref(\y_l\mid\x)}
    \right)\right].
\end{equation}
Assume:
\begin{enumerate}
    \item There is \textbf{no cyclic ranking} in $D_\mathrm{pref}$.
    \item $\forall (\x,\y_w,\y_l)\in D_\mathrm{pref}$, $\pi^\prime(\y_w\mid\x)>0$, $\pi^\prime(\y_l\mid\x)>0$,
    $\piref(\y_w\mid\x)>0$, and $\piref(\y_l\mid\x)>0$.
\end{enumerate}
If there exists a response  $\y^\prime$ sampled from a non-optimal policy $\pi^\prime$ (i.e., $J(\pi^\prime)<J(\pi^*)$ in \cref{eq:obj}), and the ranking order between $\y^*$ and $\y^\prime$ \textbf{cannot be inferred} from $D_\mathrm{pref}$, then there exists a policy $\pi^\prime$, for any $\epsilon>0$, we have $L_\mathrm{DPO}(\pi^\prime)<\epsilon$ and $\pi^\prime (\y^\prime\mid\x)>\pi^\prime(\y^*\mid\x)$.
\end{corollary}

\begin{proof}
According to \cref{eq:closeform-sol} and \cref{eq:rwd-less_eps}, $L_\mathrm{DPO}(\pi^\prime)<\epsilon$ translates to
\begin{equation}
    \log\frac{\pi^\prime(\y_w\mid\x)}{\pi^\prime(\y_l\mid\x)}>
    \log\frac{\piref(\y_w\mid\x)}{\piref(\y_l\mid\x)}+\frac{\eta}{\beta},\,\,\,\,
    \forall\,(\x,\y_w,\y_l)\in D_\mathrm{pref}.
\end{equation}
Consider the following linear programming,
\begin{align}
    \max&\,\, \log{\pi^\prime(\y^\prime\mid\x)} - \log{\pi^\prime(\y^*\mid\x)}\\
    \mathrm{s.t.}&\,\,\log{\pi^\prime(\y^i_w\mid\x^i)} - \log{\pi^\prime(\y^i_l\mid\x^i)}>
    \log\frac{\piref(\y^i_w\mid\x^i)}{\piref(\y^i_l\mid\x^i)}+\frac{\eta}{\beta},\,\,\,\,
    \forall\,(\x^i,\y^i_w,\y^i_l)\in D_\mathrm{pref}.\notag
\end{align}
Following the same proof-by-contradiction in \Cref{thm:dpo}, we can know that the above linear programming can derive unbounded positive solutions.
\end{proof}

==> tables/hh_dpo_relabel.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{ccccc}
\toprule
 & DPO & DPO + relabeling & DPO-Iter (model-generated+ relabeling) & PPO \\
\midrule
OpenAssistant Reward & 0.611 & 0.639 & 0.678 & 0.718 \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{\rebuttal{Results of relabelling the preference dataset with trained reward for DPO on HH-RLHF dataset. We observe that relabeling the preference dataset with the learned reward model enhances DPO’s performance. We hypothesize that the performance improves because a learned reward model offers a clearer training signal for DPO. Additionally, in DPO-Iter, we label the model-generated samples with the learned reward model to form the preference dataset. We observe that DPO-iter can further enhance DPO’s performance.}}
\vspace{-3mm}
\label{tab:dpo-relabel}
\end{table}
